Knoll: Creating a Knowledge Ecosystem for Large Language Models

Large language models are designed to encode general purpose knowledge about the world from Internet data. Yet, a wealth of information falls outside this scope -- ranging from personal preferences to organizational policies, from community-specific advice to up-to-date news -- that users want models to access but remains unavailable. In this paper, we propose a knowledge ecosystem in which end-users can create, curate, and configure custom knowledge modules that are utilized by language models, such as ChatGPT and Claude. To support this vision, we introduce Knoll, a software infrastructure that allows users to make modules by clipping content from the web or authoring shared documents on Google Docs and GitHub, add modules that others have made, and rely on the system to insert relevant knowledge when interacting with an LLM. We conduct a public deployment of Knoll reaching over 200 users who employed the system for a diverse set of tasks including personalized recommendations, advice-seeking, and writing assistance. In our evaluation, we validate that using Knoll improves the quality of generated responses.

==> Figures/Embeddings.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lrr}
    \toprule 
    Embedding Type &  Recall\\
    \midrule
    \texttt{all-MiniLM-L6-v2} & 0.59 \\ 
    \texttt{all-mpnet-base-v2} & 0.68 \\
    \texttt{msmarco-distilbert-cos-v5} & 0.75 \\
    \texttt{text-embedding-3-small} & 0.74 \\
    \textbf{\texttt{voyage-3-lite}} & \textbf{0.76} \\ 
    \bottomrule 
    \end{tabular}
    \caption{texttt{voyage-3-lite} embeddings offer both high recall and low latency. We compare different embedding models on module recall over our test set of 100 queries and average latency (ms) over five prompts sent to ChatGPT.}
    \label{tab:embeddings}
\end{table}

==> Sections/Intro.tex <==
Large language models (LLMs) are pre-trained on wide swathes of Internet data, allowing them to encode general-purpose knowledge about the world in its parameters~\cite{petroni2019language,roberts2020much}. While this approach has led to impressive gains on benchmarks, in real-world applications, these models still often fall short~\cite{ji2023survey,kandpal2023large,feng2024knowledge}. For example, if we want to use an LLM to answer questions about completing a CS PhD at a specific university, off-the-shelf models can generate plausible but likely generic and even hallucinated answers. However, these models are unable to handle more context-specific queries, such as when students in the program typically finish their qualifying exams, what courses best fulfill the program requirements, or where to find the best free food on campus. This shortcoming is indicative of a knowledge gap issue as models do not have access to information which may be underrepresented or unavailable altogether at training time~\cite{kasai2023realtime,vu2024freshllms,kandpal2023large}. 

Existing work has proposed technical methods for augmenting LLMs with additional external knowledge. Retrieval-based methods allow models to access an external knowledge base and provide relevant information as context~\cite{lewis2020retrieval}. These methods have been successfully employed across a diverse set of knowledge-intensive tasks, such as handling open-domain question answering~\cite{guu2020retrieval,borgeaud2022improving} or utilizing on domain-specific corpora~\cite{xiong2024benchmarking,wiratunga2024cbr,kang2024biospark}. There are also commercial offerings, such as Open AI’s Custom GPT~\cite{customgpt} or Anthropic’s Claude Projects~\cite{claude}, which allow users to create separate customized models tailored for a particular task. 

In this work, we propose an alternative vision in which end-users have access to an \emph{ecosystem of knowledge modules} that can be used to augment LLMs with contextually specific information (Fig.~\ref{fig:teaser}). We define a ``knowledge module'' as a self-contained repository of information that an individual wants their LLM to access. The ecosystem consists of two components:~(1) knowledge creators who make modules either for personal purposes or for the broader community usage and~(2) knowledge consumers who import created modules when interacting with LLMs. This ecosystem can exist at different scales, ranging from a single user creating and consuming personalized modules to a broader community where modules are maintained and shared across many users.


Our approach addresses two core problems of existing solutions for integrating customized knowledge into LLMs. First, on the knowledge creation side, current methods assume that the knowledge users want to add is readily accessible. In reality, this knowledge is likely to be diffuse --- fragmented across different sources~\cite{bernstein2008information,jones2007personal,oulasvirta2007mobile} or distributed across different people~\cite{tsoukas1996firm,hutchins2000distributed}. To address this, we support module creation from the bottom-up, allowing users to iteratively add to their modules as part of their everyday workflow and access modules that others in the communities have created. Second, for knowledge usage, the current paradigm forces users to make siloed spaces for each of their customized models~\cite{customgpt,claude}. However, this approach grows cumbersome as the number of desired use cases grows or even as the knowledge a user wants to access overlaps across models. Instead, we propose that knowledge usage should occur automatically: rather than having the user navigate to a separate workspace, the model should select the appropriate modules from the options that the user has added and utilize any relevant knowledge at inference-time. 

We instantiate this idea as software infrastructure, \emph{Knoll}, which allows users to store any information they may want a language model to have access to in the form of knowledge modules and provides relevant knowledge as context when the user is interacting with commercial language models (e.g., ChatGPT, Claude). Users are able to create new modules by clipping any text they come across on the Internet or by importing existing documents. Then, when a user queries a language model, Knoll will automatically select which modules are useful for answering the prompt. With Knoll, users also have the flexibility to select or de-select modules depending on their query and refresh the modules' contents to ensure that the knowledge being added is up-to-date. 

To evaluate Knoll, we conduct a public deployment of our infrastructure. During a two-month period, over 200 users have downloaded Knoll, sending 1,500+ queries with information added from knowledge modules. Users imported XX unique modules and created nine new modules, spanning both personal use (e.g., study guides, job applications) and community-oriented information (e.g., course policies, paper writing norms). Using data collected from our public deployment, we first conduct a technical evaluation of Knoll using a subset of 100 queries to test whether adding knowledge modules improves the quality of generated responses. We find that annotators prefer responses generated with Knoll over baseline \texttt{GPT-4o} responses for 81.5\% of the queries when external knowledge is needed. Second, we triangulate between log data (N=20X), survey responses (N=17), and semi-structured interviews (N=8) to analyze usage patterns. We find that Knoll ameliorates a data void issue, empowering users to ask queries to LLMs they otherwise would not have due to hallucinations or a lack of relevant information. 

Taken together, we introduce the concept of a modular knowledge ecosystem in which users can create, collaborate, and configure custom knowledge for their language module. We develop software infrastructure that supports this ecosystem, evaluate its ability to improve the quality of model generations, and then deploy our system for real-world usage.  



